On Bessel's Correction: Unbiased Sample Variance, the Bariance, and a Novel Runtime-Optimized Estimator

Bessel's correction adjusts the denominator in the sample variance formula from n to n-1 to ensure an unbiased estimator of the population variance. This paper provides rigorous algebraic derivations geometric interpretations and visualizations to reinforce the necessity of this correction. It further introduces the concept of Bariance an alternative dispersion measure based on pairwise squared differences that avoids reliance on the arithmetic mean. Building on this we address practical concerns raised in Rosenthals article [Rosenthal, 2015] which advocates for n-based estimates from a mean squared error (MSE) perspective particularly in pedagogical contexts and specific applied settings. Finally, the empirical component of this work based on simulation studies demonstrates that estimating the population variance via an algebraically optimized Bariance approach can yield a computational advantage. Specifically the unbiased Bariance estimator can be computed in linear time resulting in shorter runtimes while preserving statistical validity.

==> bariance_legacy.tex <==
\section{Introducing the \textit{Bariance} and an optimized linear Estimator}
We define the \textbf{\textit{Bariance}} of a sample \( \{X_1, X_2, \dots, X_n\} \) as the average squared difference over all unordered pairs:

\[
\text{\textit{Bariance}} := \frac{1}{n(n-1)} \sum_{i \ne j} (X_i - X_j)^2
\]

\noindent This can be interpreted as the average squared length of all edges in the complete graph on the sample points.

\noindent \textbf{We begin by expanding the inner squared difference}:

\[
(X_i - X_j)^2 = X_i^2 - 2X_i X_j + X_j^2
\]

\noindent Summing over all distinct \( i \ne j \):

\[
\sum_{i \ne j} (X_i - X_j)^2 
= \sum_{i \ne j} (X_i^2 + X_j^2 - 2X_i X_j)
\]

\noindent We split this into three terms:

\[
= \sum_{i \ne j} X_i^2 + \sum_{i \ne j} X_j^2 - 2 \sum_{i \ne j} X_i X_j
\]

\noindent Note the following observations:
- For fixed \( i \), there are \( n-1 \) values of \( j \ne i \), so:
  \[
  \sum_{i \ne j} X_i^2 = (n - 1) \sum_{i=1}^n X_i^2
  \]
  Similarly, \( \sum_{i \ne j} X_j^2 = (n - 1) \sum_{j=1}^n X_j^2 \)

\noindent So the first two terms become:
\[
\sum_{i \ne j} X_i^2 + \sum_{i \ne j} X_j^2 = 2(n-1) \sum_{i=1}^n X_i^2
\]

\noindent Now consider the double sum:
\[
\sum_{i \ne j} X_i X_j = \left( \sum_{i=1}^n \sum_{j=1}^n X_i X_j \right) - \sum_{i=1}^n X_i^2
= \left( \sum_{i=1}^n X_i \right)^2 - \sum_{i=1}^n X_i^2
\]

\noindent Combine:

\[
\sum_{i \ne j} (X_i - X_j)^2
= 2(n-1) \sum X_i^2 - 2\left( \left( \sum X_i \right)^2 - \sum X_i^2 \right)
\]

\[
= 2(n-1) \sum X_i^2 - 2\left( \left( \sum X_i \right)^2 - \sum X_i^2 \right)
= 2(n-1) \sum X_i^2 - 2 \left( \sum X_i \right)^2 + 2 \sum X_i^2
\]

\[
= 2n \sum X_i^2 - 2 \left( \sum X_i \right)^2
\]

\noindent \textbf{Substitute back into the \textit{Bariance} formula}. Now divide by \( n(n-1) \):

\[
\text{\textit{Bariance}} = \frac{1}{n(n-1)} \sum_{i \ne j} (X_i - X_j)^2
\equiv \frac{2n}{n(n-1)} \sum X_i^2 - \frac{2}{n(n-1)} \left( \sum X_i \right)^2
\]
See empirical verification in appendix A.

\[
\boxed{
\text{\textit{Bariance}} = \frac{2}{n - 1} \left(\sum X_i^2 \right)
- \frac{2}{n(n - 1)} \left( \sum X_i \right)^2
}
\]

\subsection{In the Case Of Mean-centered data}

\noindent If the data is centered, i.e., \( \sum X_i = 0 \), then:

\[
\text{\textit{Bariance}} = \frac{2n}{n(n - 1)} \sum X_i^2 = \frac{2}{n - 1} \sum X_i^2
\]

\noindent We now relate this to the unbiased sample variance:

\[
\hat{S}^2 = \frac{1}{n - 1} \sum_{i=1}^n (X_i - \bar{X})^2
= \frac{1}{n - 1} \sum X_i^2 \quad \text{(since } \bar{X} = 0 \text{)}
\]

\noindent Therefore, following equality holds for the defined ``\textit{Bariance}``:

\[
\boxed{
\text{\textit{Bariance}} = 2 \cdot \hat{S}^2
}
\]

\noindent This result shows that \textit{Bariance} represents twice the unbiased sample variance when the sample is mean-centered. It provides an elegant \textbf{pairwise perspective} on variance: instead of summing squared deviations from a central value, we sum squared differences between all pairs and average, regardless of the reference point within the sample.

\subsubsection{Estimator Comparison in the case of mean-centered data}

Let \( \theta = \sigma^2 = 1 \). Then:
\[
\begin{aligned}
\mathbb{E}[\hat{S}^2] &= \theta \\
\mathbb{E}[\text{\textit{Bariance}}] &= 2\theta \\
\text{Bias}(\hat{S}^2) &= 0 \\
\text{Bias}(\text{\textit{Bariance}}) &= \theta \\
\text{Var}(\text{\textit{Bariance}}) &= 4 \cdot \text{Var}(\hat{S}^2) \\
\text{MSE}(\hat{S}^2) &= \text{Var}(\hat{S}^2) \\
\text{MSE}(\text{\textit{Bariance}}) &= 4 \cdot \text{Var}(\hat{S}^2) + \theta^2
\end{aligned}
\]


Subsequent, Numerical Verification of Theoretical Relationships with  
\( n = 100 \) and $\tau = 1000$:
\[
\text{Var}(\hat{S}^2) = 0.01988, \quad
\text{Var}(2 \cdot \hat{S}^2) = 0.07951
\]
\[
\text{MSE}(\hat{S}^2) = 0.02151, \quad
\text{MSE}(2 \cdot \hat{S}^2) = 1.0832
\]
\[
4 \cdot \text{Var}(\hat{S}^2) = 0.07951 \quad \Rightarrow \quad
\text{Var identity approximately holds}
\]
\[
4 \cdot \text{Var}(\hat{S}^2) + \theta^2 = 0.07951 + 1 = 1.07951 \quad \Rightarrow \quad
\text{MSE identity approximately holds}
\]
\[
\boxed{
\begin{aligned}
\text{Var}(2 \cdot \hat{S}^2) &= 4 \cdot \text{Var}(\hat{S}^2) \\
\text{MSE}(2 \cdot \hat{S}^2) &= 4 \cdot \text{Var}(\hat{S}^2) + \theta^2
\end{aligned}
}
\]


\noindent \textbf{Main Findings}:

\begin{itemize}
    \item \( \hat{S}^2 \): unbiased, lower MSE, standard estimator.
    \item \textit{Bariance}: biased (by \( +\theta \)), higher MSE due to both variance inflation and squared bias.
    \item Useful relation: \( \text{\textit{Bariance}} = 2 \cdot \hat{S}^2 \)
\end{itemize}

Numerically (for \( n = 100 \), $\mathcal{N}(0,1)$, $\tau$=1000):

\vspace{0.5em}

\begin{center}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Estimator} & \textbf{Point Estimate} & \textbf{Bias} & \textbf{Variance} & \textbf{MSE} \\
\hline
Unbiased sample variance & 1.00091 & 0.00091 & 0.02156 & 0.02151 \\
\textit{Bariance} & 2.00181 & 1.00181 & 0.08625 & 1.08968 \\
\hline
\end{tabular}
\end{center}

\newpage


\subsection{A Short Numerical Example with Five Numbers}

Let \( X = \{2, 4, 6, 8, 10\} \), so the sample mean is:
\[
\bar{X} = \frac{2 + 4 + 6 + 8 + 10}{5} = 6
\]

The sum of squared deviations:
\[
\sum_{i=1}^5 (X_i - \bar{X})^2 = (2{-}6)^2 + (4{-}6)^2 + (6{-}6)^2 + (8{-}6)^2 + (10{-}6)^2 = 16 + 4 + 0 + 4 + 16 = 40
\]

Unbiased sample variance:
\[
\hat{S}^2 = \frac{1}{n - 1} \sum_{i=1}^n (X_i - \bar{X})^2 = \frac{40}{4} = 10
\]

Biased sample variance:
\[
S^2_{\text{biased}} = \frac{1}{n} \sum_{i=1}^n (X_i - \bar{X})^2 = \frac{40}{5} = 8
\]

The sum of all pairwise squared differences:
\[
\sum_{i < j} (X_i - X_j)^2 = 16 + 4 + 0 + 4 + 16 + 36 + 64 + 36 + 4 + 4 = 200
\]

\textit{Bariance}:
\[
\text{\textit{Bariance}} = \frac{1}{n(n-1)} \sum_{i < j} (X_i - X_j)^2 = \frac{200}{20} = 10
\quad \Rightarrow \quad \boxed{\text{\textit{Bariance}} = 2 \cdot \hat{S}^2}
\]

\subsubsection*{Summary Table of Point Estimators}

\begin{center}
\begin{tabular}{|l|c|}
\hline
\textbf{Metric} & \textbf{Value} \\
\hline
Sample Mean \( \bar{X} \) & 6 \\
Variance (biased) \( S^2_{\text{biased}} \) & 8 \\
Variance (unbiased) \( \hat{S}^2 \) & 10 \\
\textit{Bariance} & 20 \\
\textit{Bariance} / 2 & 10 \\
\hline
\end{tabular}
\end{center}



\subsection{Graph-Theoretic View of \textit{Bariance}}

\begin{center}
\begin{tikzpicture}[scale=1.2]
\coordinate (X1) at (1,1);
\coordinate (X2) at (2.5,2.2);
\coordinate (X3) at (4,1);
\coordinate (X4) at (3.5,0);
\coordinate (X5) at (2,0.3);

\foreach \pt/\lbl in {X1/$X_1$, X2/$X_2$, X3/$X_3$, X4/$X_4$, X5/$X_5$} {
  \draw[fill=black] (\pt) circle (1.5pt);
  \node at ($( \pt ) + (0.2, 0.2)$) {\lbl};
}

\foreach \i/\j in {X1/X2, X1/X3, X1/X4, X1/X5,
                   X2/X3, X2/X4, X2/X5,
                   X3/X4, X3/X5,
                   X4/X5}
  \draw[gray!50, dashed] (\i) -- (\j);
\end{tikzpicture}
\captionof{figure}{Complete graph over sample points. Each edge represents a pairwise squared difference that contributes to the \textit{ bariance}.}
\end{center}
Each dashed edge on the graph corresponds to a pair \( (X_i, X_j) \), and the squared difference \( (X_i - X_j)^2 \) can be viewed as an edge weight. Since the graph is fully connected (a complete graph \( G_n \)), there are \( \binom{n}{2} \) such edges.

\noindent From a graph-theoretic standpoint,\textit{ bariance} is the \textbf{average squared edge length} of the complete weighted graph over the sample. In this context:\\
\noindent- Nodes = observations \( X_i \) \\
- Edges = pairwise differences \\
- Weights = squared differences \( (X_i - X_j)^2 \)

\noindent This perspective connects naturally to \textbf{distance-based dispersion measures} in statistical graph theory, including energy statistics and certain U-statistics. It also provides an intuitive, coordinate-free alternative to the variance's reliance on a central location (i.e., the mean).





\subsection{Deviation from Mean (Variance) vs. Pairwise Differences (\textit{Bariance})}

\begin{center}
\begin{tikzpicture}
\draw[->] (0,0) -- (11,0) node[right] {$X$};

\foreach \x/\label in {2/$X_1$, 4/$X_2$, 6/$X_3$, 8/$X_4$, 10/$X_5$}
  \draw[fill=black] (\x,0) circle (2pt) node[below] {\label};

\draw[dashed, red] (6,0) -- (6,2.2) node[above] {\textcolor{red}{$\bar{X} = 6$}};
\foreach \x/\h in {2/0.4,4/0.6,8/0.8,10/1.0}
  \draw[<->, blue] (\x,\h) -- (6,\h);

\draw[<->, green!60!black, thick] (2,1.6) -- (10,1.6) node[midway, above] {\scriptsize $X_5 - X_1$};
\end{tikzpicture}
\captionof{figure}{Blue: variance (mean-deviation, n-1 degrees of freedom adjustment). Green: pairwise distance = a \textit{Bariance} component.}
\end{center}


\subsection{The Pairwise Difference Grid}

\begin{center}
\begin{tikzpicture}
\foreach \i in {0,...,4} {
    \foreach \j in {0,...,4} {
        \pgfmathsetmacro\val{(2*\i - 2*\j)^2}
        \node at (\j, -\i) {\val};
    }
}
\draw[step=1cm, transparent, very thin] (0,-4) grid (4,0);
\foreach \i/\val in {0/2,1/4,2/6,3/8,4/10} {
    \node at (-1.5,-\i) {\val};
    \node at (\i, 0.5) {\val};
}
\end{tikzpicture}
\captionof{figure}{Symmetric matrix of squared pairwise differences \( (X_i - X_j)^2 \) for \( X = \{2, 4, 6, 8, 10\} \). Diagonal elements are zero (self-distances).}
\end{center}

\noindent This matrix visualizes all pairwise squared differences between elements of \( X \). Its key properties:\\

\noindent - Symmetry: \( (X_i - X_j)^2 = (X_j - X_i)^2 \), so the grid is symmetric across the main diagonal.\\
- Diagonal: Always zero, since \( (X_i - X_i)^2 = 0 \).\\
- Off-diagonal structure: Each non-zero entry contributes to the total in the \textit{Bariance} calculation.\\

\noindent  This grid-based view reinforces how the redundancy in the pairwise differences allows us to simplify the computation algebraically. Instead of evaluating all \( n(n - 1) \) pairs, we can summarize the matrix using aggregate row/column sums, which enables the linear-time optimized formula for the \textit{Bariance}:
\[
\text{\textit{Bariance}} = \frac{2n}{n(n-1)} \sum X_i^2 - \frac{2}{n(n-1)} \left( \sum X_i \right)^2
\]

\noindent Thus, symmetry is not just a visual feature—it underpins the algebraic transformation that reduces the quadratic computational complexity to linear.


\newpage


\newpage

\subsection{On the Estimator Performance of the \textit{Bariance} Point Estimator using $\Gamma$-distributed Data}

Let \( X \sim \text{$\Gamma$}(k = 2, \theta = 2) \Rightarrow \mathbb{E}[X] = 4, \quad \text{Var}(X) = 8 \), Using \( n = 100 \), $\tau = 1000$ we obtain:

\subsubsection*{Summary Table of Empirical \textit{Bariance} Point Estimator Performance}

\begin{center}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Estimator} & \textbf{Mean} & \textbf{Bias} & \textbf{Variance} & \textbf{MSE} \\
\hline
Unbiased Sample Variance Estimator & 8.00087 & 0.00087 & 2.92574 & 2.92281 \\
\( \text{\textit{Bariance}} \) & 16.00174 & 8.00174 & 11.70295 & 75.71907 \\
\hline
\end{tabular}
\end{center}

\subsubsection*{Numerical Verification of Theoretical Relationships}

Let \( \sigma^2 = 8 \Rightarrow \sigma^4 = 64 \):

\[
\text{Var}(\hat{S}^2) = 2.92574, \quad
\text{Var}(\text{\textit{Bariance}}) = 11.70295
\]
\[
\text{Empirical MSE}(\text{\textit{Bariance}}) = 75.71907
\]

We numerically verify:

\[
\text{Var}(\text{\textit{Bariance}}) \approx 4 \cdot \text{Var}(\hat{S}^2)
\quad \Rightarrow \quad
11.70295 \approx 4 \cdot 2.92574 = 11.70296
\]
\[
\text{MSE}(\text{\textit{Bariance}}) \approx 4 \cdot \text{Var}(\hat{S}^2) + \sigma^4
\quad \Rightarrow \quad
75.71907 \approx 4 \cdot 2.92574 + 64 = 75.70295
\]
\[
\text{Relations hold numerically with high accuracy:} \quad
\begin{cases}
\text{Var}(\text{\textit{Bariance}}) = 4 \cdot \text{Var}(\hat{S}^2) \\
\text{MSE}(\text{\textit{Bariance}}) = 4 \cdot \text{Var}(\hat{S}^2) + \sigma^4
\end{cases}
\]


==> notation_table.tex <==
\begin{table}[h!]
\centering
\caption{Notation Reference for Variance Estimation and \textit{Bariance} Formulas}
\label{tab:notation}
\begin{tabular}{ll}
\toprule
\textbf{Symbol} & \textbf{Description} \\
\midrule
$\bar{X}$ & Sample mean \\
$S^2$ & Biased sample variance estimator (denominator $n$) \\
$\hat{S}^2$ & Unbiased sample variance estimator (Bessel-corrected, denominator $n-1$) \\
$\text{\textit{Bariance}}$ & Naïve pairwise estimator of variance over all unordered pairs \\
$\text{\textit{Bariance}}_{\text{opt}}$ & Optimized algebraic formula for the \textit{Bariance} \\
$\sigma^2$ & True population variance \\
$\text{Bias}(\hat{\theta})$ & Bias of an estimator \\
$\text{Var}(\hat{\theta})$ & Variance of an estimator \\
$\text{MSE}(\hat{\theta})$ & Mean squared error of an estimator \\
$\sum_{i \ne j} (X_i - X_j)^2$ & Total of all pairwise squared differences in the sample \\
$\sum X_i$ & Sum of all sample values \\
$\sum X_i^2$ & Sum of squared sample values \\
\bottomrule
\end{tabular}
\end{table}


==> old_java_runtime_analysis_section.tex <==
\section{Robustness Check of Empirical Runtime in Java SE}

To verify the consistency of results across platforms, we implemented both the Unbiased and Optimized Bariance estimators in \textbf{Java 21.0.1} on a system with the following configuration:

\begin{itemize}
  \item \textbf{Operating System:} Mac OS X 13.0
  \item \textbf{Architecture:} \texttt{aarch64}
  \item \textbf{Cores Available:} 10 (used single-threaded)
  \item \textbf{Max Memory:} 4 GB (JVM-reported)
\end{itemize}

\subsection*{Runtime Results}

\subsection{Normal-distributed data}

Each estimator was benchmarked over 100 trials for each sample size. Figure~\ref{fig:java-candle} shows the mean runtime with 95\% confidence intervals for both estimators.



\begin{figure}[h!]
\centering
\includegraphics[width=0.95\textwidth]{java/output (6).png}
\caption{Candlestick plots (mean $\pm$ 1.96 SE) of Java runtime estimates for Unbiased and Optimized Bariance estimators.}
\label{fig:java-candle}
\end{figure}

\subsection*{Density of Estimates}

Figure~\ref{fig:java-density} shows the distribution of runtime for each estimator across selected sample sizes, visualized via kernel density estimates.

\begin{figure}[h!]
\centering
\includegraphics[width=0.95\textwidth]{java/java_density_fixed.png}
\caption{Density plots of runtime for Unbiased and Optimized Bariance estimators in Java, stratified by sample size.}
\label{fig:java-density}
\end{figure}

\clearpage
\newpage

\subsection{$\Gamma$(2.0, 2.0)-distributed Data}

\begin{figure}[ht]
\centering
\includegraphics[width=0.95\textwidth]{runtime_density_gamma_1k_grid_display__BEST_SO_FAR.png}
\caption{
Kernel density estimates of runtime (in nanoseconds) for the \texttt{Unbiased} and \texttt{BarianceOpt} variance estimators across nine increasing sample sizes (from $n=100$ to $n=500{,}000$).
Each panel is based on 1,000 trials using data sampled from a $\Gamma(2.0, 2.0)$ distribution. 
Vertical dashed lines indicate the mean runtime per estimator and sample size.
This visualization highlights the increasingly efficient runtime of \texttt{BarianceOpt} relative to \texttt{Unbiased} as $n$ grows large.
}
\label{fig:runtime_density_comparison}
\end{figure}



\begin{figure}[ht]
\centering
\includegraphics[width=0.95\textwidth]{FAST_5_GAMMA_DIST_GUCCI_Plot.png}
\caption{
Estimated mean runtimes (nanoseconds) for five variance estimators across six sample sizes. 
Each point reflects the mean runtime estimated from 1,000 Monte Carlo trials using Java's \texttt{System.nanoTime()}. 
Error bars represent 95\% confidence intervals obtained from a fixed effects OLS regression on sample size and estimator.
Data were generated from a $\Gamma(2.0, 2.0)$ distribution with fixed seed (42). 
Classical estimators include the biased and unbiased sample variance and the population variance. 
\textit{Bariance}-based methods refer to the optimized and alternative scalar formulations detailed in Section~\ref{sec:notation}.
Pairwise estimators were excluded due to high computational cost. See Table~\ref{tab:runtime_ols} for regression coefficients.
}
\label{fig:runtime_benchmark}
\end{figure}



\begin{table}[ht]
\centering
\caption{OLS Regression of Runtime on Estimator and Sample Size}
\label{tab:runtime_ols}
\begin{tabular}{lrr}
\hline
 & Coefficient & Std. Error \\
\hline
Intercept                     & 698.33*** & (25.85) \\
Estimator: \texttt{BarianceOpt} & -909.21*** & (29.46) \\
Estimator: \texttt{Biased}      & -694.43*** & (28.91) \\
Estimator: \texttt{PopulationVar} & 1457.29*** & (25.56) \\
Estimator: \texttt{Unbiased}     & -690.49*** & (28.98) \\
Sample Size = 500             & 229.27*** & (27.55) \\
Sample Size = 1000            & 534.47*** & (29.38) \\
Sample Size = 2000            & 800.55*** & (31.78) \\
Sample Size = 3000            & 1656.77*** & (31.82) \\
Sample Size = 5000            & 2221.24*** & (32.95) \\
\hline
R-squared & \multicolumn{2}{c}{0.455} \\
Observations & \multicolumn{2}{c}{22,906} \\
\hline
\end{tabular}
\begin{flushleft}
\footnotesize \textit{Notes:}  
Dependent variable is runtime in nanoseconds. Model estimated via OLS with fixed effects for estimator and sample size. Runtime measured using Java's \texttt{System.nanoTime()}.

\textbf{Estimators (notation from Section~\ref{sec:notation}):}
\begin{itemize}
  \item \texttt{Unbiased} (\( \hat{S}^2 \)): \( \frac{1}{n - 1} \sum_{i=1}^n (X_i - \bar{X})^2 \)
  \item \texttt{Biased} / \texttt{PopulationVar} (\( S^2 \)): \( \frac{1}{n} \sum_{i=1}^n (X_i - \bar{X})^2 \)
  \item \texttt{BarianceOpt} (\( \text{\textit{Bariance}}_{\text{opt}} \)): \( \frac{2n}{n(n-1)} \sum X_i^2 - \frac{2}{n(n-1)} \left( \sum X_i \right)^2 \)
  \item \texttt{AltBariance} (alternative form): \( \frac{2}{n-1} \left[ \sum X_i^2 - \frac{1}{n} \left( \sum X_i \right)^2 \right] \)
  \item \texttt{Pairwise estimators} (excluded): \( \text{\textit{Bariance}} = \frac{1}{n(n-1)} \sum_{i \ne j} (X_i - X_j)^2 \)
\end{itemize}

Each estimator was run over 1,000 trials per sample size with data drawn from \( \Gamma(2.0, 2.0) \), seeded at 42. Pairwise estimators were excluded from regression due to excessive computational cost. All implementations validated via a synthetic test suite.

\textbf{The Benchmark Environment:}
\begin{itemize}
  \item OS: Mac OS X 13.0
  \item Architecture: \texttt{aarch64}
  \item Java Version: 21.0.1
  \item Available Processors: 10
  \item Max Memory: 4096 MB
\end{itemize}
\end{flushleft}
\end{table}




\clearpage
\newpage


==> runtime_benchmark_report.tex <==


\section*{Execution Environment}

All simulations were run in a Python environment using:
\begin{itemize}
  \item Python 3.9+
  \item NumPy, SciPy, Pandas, Matplotlib
  \item Single-threaded virtualized CPU
  \item 50 trials per sample size and estimator
\end{itemize}

\section*{Simulation Setup}

\begin{itemize}
  \item Estimators: Unbiased Variance (Vectorized) and Optimized Bariance (Vectorized)
  \item Distribution: Standard Normal $\mathcal{N}(0, 1)$
  \item Sample sizes tested: 100, 200, 300, 500, 1000, 2000
  \item Runtime measured with high-resolution wall-clock timer
\end{itemize}

\section*{Statistical Summary of Differences}

The table below reports the mean difference (Unbiased - Bariance), standard deviation (SD), $t$-statistic, $p$-value, and 95\% confidence interval.

\begin{center}
\begin{tabular}{rrrrrrr}
\toprule
Sample Size & Mean Diff & SD & $t$ & $p$ & 95\% CI Lower & Upper \\
\midrule
100 & 7.14e-06 & 3.69e-05 & 1.37 & 1.78e-01 & -3.09e-06 & 1.74e-05 \\
200 & 3.38e-06 & 1.57e-05 & 1.52 & 1.35e-01 & -9.81e-07 & 7.73e-06 \\
300 & -2.91e-06 & 9.76e-06 & -2.11 & 4.00e-02 & -5.62e-06 & -2.07e-07 \\
500 & 3.70e-05 & 2.87e-05 & 9.13 & 3.84e-12 & 2.90e-05 & 4.49e-05 \\
1000 & 2.25e-05 & 1.04e-05 & 15.28 & 2.84e-20 & 1.96e-05 & 2.54e-05 \\
2000 & 2.43e-05 & 9.42e-06 & 18.24 & 1.76e-23 & 2.17e-05 & 2.69e-05 \\
\bottomrule
\end{tabular}
\end{center}

\section*{Visualization}

\begin{figure}[h!]
\centering
\includegraphics[width=0.8\textwidth]{difference_plot.png}
\caption{Mean Runtime Difference (Unbiased - Bariance) with 95\% Confidence Interval (in microseconds)}
\end{figure}



==> runtime_table.tex <==
% latex table generated in R 4.3.1 by xtable 1.8-4 package
% Fri May 23 00:31:01 2025
\begin{table}[ht]
\centering
\begin{tabular}{rrlrr}
  \hline
 & SampleSize & Estimator & Mean\_Runtime\_s & SD \\ 
  \hline
1 & 20.000000 & Bariance\_Naive & 0.000170 & 0.000587 \\ 
  2 & 20.000000 & Bariance\_Opt & 0.000080 & 0.000442 \\ 
  3 & 20.000000 & Biased & 0.000130 & 0.000562 \\ 
  4 & 20.000000 & Unbiased & 0.000050 & 0.000219 \\ 
   \hline
\end{tabular}
\end{table}

